Private Cross-Silo Federated Learning for Extracting Vaccine Adverse Event Mentions

Federated Learning (FL) is quickly becoming a goto distributed training paradigm for users to jointly train a global model without physically sharing their data. Users can indirectly contribute to, and directly benefit from a much larger aggregate data corpus used to train the global model. However, literature on successful application of FL in real-world problem settings is somewhat sparse. In this paper, we describe our experience applying a FL based solution to the Named Entity Recognition (NER) task for an adverse event detection application in the context of mass scale vaccination programs. We present a comprehensive empirical analysis of various dimensions of benefits gained with FL based training. Furthermore, we investigate effects of tighter Differential Privacy (DP) constraints in highly sensitive settings where federation users must enforce Local DP to ensure strict privacy guarantees. We show that local DP can severely cripple the global model's prediction accuracy, thus dis-incentivizing users from participating in the federation. In response, we demonstrate how recent innovation on personalization methods can help significantly recover the lost accuracy. We focus our analysis on the Federated Fine-Tuning algorithm, FedFT, and prove that it is not PAC Identifiable, thus making it even more attractive for FL-based training.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> fedmoe.tex <==
\section{Federated Mixture-of-Experts (\fedmoe)}

%\section{Model Definition}

At its core, our proposal is to mix the outputs of a
collaboratively-learned general model and a local domain expert model.
Participating users have their independent set of labeled training
examples that they wish to keep private, drawn from user-specific
domain distributions.  These users collaborate to build a general
model for the task.  At the same time, users maintain private,
domain-adapted expert models.
%\ref{fig:fl-de-picture} depicts the FL setting with one private
%domain expert for each user.
The final predictor for each user is a weighted average of the outputs from the
general and private models.  These weights are learned using a MoE
architecture~\cite{masoudnia14,nowlan1991}, so the entire model can be
trained with gradient descent.

%A user's domain expert model can converge to the general model if the
%user's data distribution has a significant overlap with the data
%distributions of other users.  If however, the user's data
%distribution is significantly different from other users, its domain
%expert model will likely diverge from the general model.

\begin{figure}
%\ffigbox{\TopFloatBoxes
\includegraphics[width=\columnwidth]{figures/fl-de-picture}
%}{
\caption{The Federated Learning setting with Domain Experts, one per
  participating user.  Each user uses its local MoE combination model for both
  training and inference.}
\label{fig:fl-de-picture}
%}
%\end{floatrow}
\end{figure}

%Figure \ref{fig:fl-de-picture} depicts our overall system architecture. 
Our overall system architecture follows.
$M_G$ is the general model that is trained by the FL
framework.  $(\varepsilon,\delta)$-differential privacy is enforced by
clipping gradients and adding noise to the gradients sent back to the federation server.
Each of the $i$ users maintains a private model, $M_{P_i}$, which act as 
domain experts tuned to the respective users'
data distributions.  A user uses its private labeled data to retrain
its private model $M_{P_i}$ along with $M_G$.  $M_{P_i}$ is completely
private to the user and hence does not need DP-inducing noise.  The
MoE framework at each user combines outputs of the two models, tuning
the MoE output to better suit the user's data distribution if needed.

More formally, let $M_G$ be a general model, with parameters
$\Theta_G$, so that $\hat{y}_{G} = M_G(x, \Theta_G)$ is $M_G$'s
predicted probability for the positive class, or perhaps a regressed
value\footnote{Although we tested only binary classification and
  regression in our experiments, there are obvious extensions to
  multiclass problems.}.  $M_G$ is shared between all users, and is
trained on all data using FL with differentially private
SGD~\cite{abadi16}, enabling each user to contribute to training the
general model\footnote{Because $M_G$ is trained using DP SGD protocols,
we can guarantee differential privacy of the model $M_G$. No data besides
these differentially-private gradients is ever sent over public channels,
so our architecture guarantees differential privacy for anyone without access
to the private models $M_{P_i}$.}.

Similarly, let $M_{P_i}$ be a private model of user $i$, parameterized
by $\Theta_{P_i}$, and $\hat{y}_{P_i} = M_{P_i}(x, \Theta_{P_i})$ be
the model's predicted probability. Although $M_{P_i}$ could have a
different architecture from $M_G$, in this work we initialize
$M_{P_i}$ as an exact copy of $M_G$. Neither $M_{P_i}$, nor gradient
information about it, is shared with any other party, so $M_{P_i}$ can
be updated exactly, without including privacy-related noise.

These two models are combined using a \emph{gating function},
$\alpha_i(x)$, that can learn which model to trust as a function of
the input.  In our experiments, we set $\alpha_i(x) = S(w_i^{T}
\cdot x + b_i)$, where $S(x)$ is the sigmoid function, and $w_i$ and
$b_i$ are learned weights.  Although there are many other choices for
the gating function, this choice is simple, differentiable, and allows
smooth mixing across the boundary between the two models.
%% This gating function essentially
%% learns which regions to trust the private model over the general
%% model, and allows smooth mixing along the boundary.  Thus the final
%% output $\hat{y_i}$ depends on learned parameters $\Theta_G$,
%% $\Theta_{P_i}$, $w_i$, and $b_i$, and all are updated via SGD.

Thus the final output
$\hat{y_i}$ depends on learned parameters $\Theta_G$, $\Theta_{P_i}$,
$w_i$, and $b_i$, and all are updated via SGD.
The final output that user $i$ uses to label data is
\begin{equation}
  \hat{y}_i = \alpha_i(x) M_G(x, \Theta_G) + (1 - \alpha_i(x)) M_{P_i} ( x, \Theta_{P_i}).
  \label{eq3}
\end{equation}

We advise, in line with standard MoE practice, that the training of the gating function
parameters is separated from the training of the training of the expert models themselves.
In all experiments, we split the training data in two and train the parameters of $\alpha_i(x)$ separately
from the models $M_G$ and $M_{P_i}$. We call this held-out data $H_t$ in the pseudocode below.

\begin{algorithm}[t]

  \begin{algorithmic}[1]
    
    \REQUIRE User $i$, their $N$ examples ${x_1,x_2,\ldots,x_N}$ and
    corresponding labels ${y_1, y_2, \ldots, y_N}$, along with labeled
    held out examples $H_t$ to train the gating function, general
    model $M_G$ and its parameters $\Theta_G$, private model $M_{P_i}$
    and its parameters $\Theta_{P_i}$, gating function $\alpha_i$ and
    its parameters $\Theta_{\alpha_i}$, learning rate $\eta_t$, noise
    scale $\sigma$, group size $L$, gradient norm bound $C$

    \STATE {\bf Initialize} ${\bf g}$, ${\bf g}_G$, ${\bf g}_{P_i}$ to $0$.
    
    \STATE Take a random sample of data, $L_t$, with sampling probability $L/N$
    \FOR{$x_t \in L_t$}
    \STATE Compute prediction $\hat{y}_t$ with equation \ref{eq3}
    \STATE Compute loss $l_t = ||y_t - \hat{y}_t||$
    \STATE ${\bf g}_G += compute\_clipped\_gradient(l_t, \Theta_G, C)$
    \STATE ${\bf g}_{P_i} += compute\_gradient(l_t, \Theta_{P_i})$
    \ENDFOR
    \STATE Take a sample of held-out data, $H_t$
    \FOR{$x_t \in H_t$}
    \STATE Compute prediction $\hat{y}_t$ with equation \ref{eq3}
    \STATE Compute loss $l_t = ||y_t - \hat{y}_t||$
    \STATE ${\bf g}_{\alpha_i} += compute\_gradient(l_t, \Theta_{\alpha_i})$
    \ENDFOR
    \STATE ${\bf g}_G += gaussian\_noise(0, C *\sigma^2)$    
    \STATE $\Theta_{P_i} \gets \Theta_{P_i} - \frac{\eta_t}{L} {\bf g}_{P_i}$
    \STATE $\Theta_{\alpha_i} \gets \Theta_{\alpha_i} - \frac{\eta_t}{L} {\bf g}_{\alpha_i}$
    
    \STATE Send ${\bf g}_G / L$ to the Federation Server.

    
  \end{algorithmic}
  \caption{Minibatch Update for Mixture of Experts at user $i$ (Outline).}
  \label{alg:1}
  
\end{algorithm}

Algorithm \ref{alg:1} depicts a single batch of MoE training for user $i$ at a high level.
During training, each user will perform this procedure many times, while
receiving updates to the general model from the federation server. The
differentially-private gradient computation ${\bf g}_G$ is based on algorithm by Abadi
et. al.~\cite{abadi16}.  We apply equation~\ref{eq3} to control the gradient
aggregate ${\bf g}$ that is eventually sent to the federation server.

The private model $M_{P_i}$ and weighting mechanism $\alpha_i$ work
together to provide a significant benefit over differentially private
FL. First, by allowing individual domain adaptation, they boost
accuracy. Second, because they allow noise-free updates, they prevent
the accuracy loss associated with more stringent privacy requirements,
which add noise to the general model.

Over time, a user's gating function
$\alpha_i(x)$ learns whether to trust the general model or the private model
more for a given input, and the private model $M_{P_i}$ needs to perform
well on only the subset of points for which the general model fails.
The failure of the general model is expected, and corrected, so the mixture
of experts can tolerate a poor-quality general model so long as it is 
reliably correct in at least some region of the input space.

\section{Effects of the Gating Function on Gradients}

One advantage of our MoE setup is that the loss is
differentiable with respect to all model parameters -
the parameters of the private and general models, and the
gating function. When $\alpha_i(x) << 1$, the general
model makes little contribution to the user's prediction.
But this gating function also gates the gradients, because
the general model makes little contribution to the loss.
Symmetrically, the gradients for the private model vanish
as $\alpha_i(x) \to 1$.

For the private model, gating the gradients is perfectly reasonable.
Once the gating function is sure that the general model is making
accurate predictions on a particular data point, there is no need to
penalize the private model for its performance in that region.  The
tradeoff in model quality is not symmetric for the shared model,
however, because the quality of the shared model affects multiple
users.  Especially if new users are joining the federation over time,
it is still desirable that the general model performs as well as
possible while satisfying privacy concerns.

On the other hand, allowing the gating function to suppress updates to
the general model may be beneficial for the privacy of user data. Once
a users' gating function has learned to trust their private model on a
particular data point, there is little incentive for them to share
further information about that data point with the federation pool.
However, if the overall quality of the general model is not a part of
the objective, it only needs to make satisfactory recommendations in a
small region of the input space, particularly the regions commonly
shared amongst several users.  Different regions of reliability
correspond to different local optima, and there are many
locally-optimal solutions where the general model is an extremely poor
model for the overall task, but is still a useful expert for most
users on some portion of inputs.  We characterize this phenomenon by
observing the behavior of the model during training, and evaluation of
the shared model on a held-out dataset.

We examine the effects of allowing the gating function to suppress
gradients by implementing an alternative algorithm, that still uses an
MoE framework.  In the modified algorithm, users compute the loss and
gradient of the general model on their data points, and send gradients
according to the DP SGD procedure, regardless of the weight
$\alpha_i(x)$. Then they compute the final prediction using the MoE,
and make noise-free updates to their private model and gating function
as before.  This makes the training of the general model equivalent to
traditional FL, while allowing the flexibility of the MoE to improve
predictions for each user. This change is implemented by computing,
in addtion to $l_t$, a loss
\[
l_t^{G} = || y_t - M_G(x_t, \Theta_G) ||,
\]
and replacing line 6 of Algorithm 1 with
\[
{\bf g}_G += compute\_clipped\_gradient(l_t^{G}, \Theta_G, C).
\]
 We refer to this modified version as Algorithm 2.

\iffalse
\begin{algorithm}[t]

  \begin{algorithmic}[1]
    
    \INPUT User $i$, their $N$ examples ${x_1,x_2,\ldots,x_N}$ and corresponding
    labels ${y_1, y_2, \ldots, y_N}$, along with labeled held out examples $H_t$
    to train the gating function, general model $M_G$ and its parameters $\Theta_G$,
    private model $M_{P_i}$ and its parameters $\Theta_{P_i}$, gating function
    $\alpha_i$ and its parameters $\Theta_{\alpha_i}$, learning rate
    $\eta_t$, noise scale $\sigma$, group size $L$, gradient norm
    bound $C$

    \STATE {\bf Initialize} ${\bf g}$, ${\bf g}_G$, ${\bf g}_{P_i}$ to $0$.
    
    \STATE Take a random sample $L_t$ with sampling probability $L/N$
    \FOR{$x_t \in L_t$}
    
    \STATE Compute prediction $\hat{y}_t$ with equation \ref{eq3}
    \STATE Compute loss $l_t = ||y_t - \hat{y}_t||$
    \STATE Compute loss $l_t^{G} = || y_t - M_G(x_t, \Theta_G) ||$
    \STATE 
    \STATE ${\bf g}_{P_i} += compute\_gradient(l_t, \Theta_{P_i})$
    \ENDFOR
    \STATE Take a sample of held-out data, $H_t$
    \FOR{$x_t \in H_t$}
    \STATE Compute prediction $\hat{y}_t$ with equation \ref{eq3}
    \STATE Compute loss $l_t = ||y_t - \hat{y}_t||$
    \STATE ${\bf g}_{\alpha_i} += compute\_gradient(l_t, \Theta_{\alpha_i})$
    \ENDFOR
    \STATE ${\bf g}_G += gaussian\_noise(0, \sigma)$
    \STATE $\Theta_{P_i} \gets \Theta_{P_i} - \frac{\eta_t}{L} {\bf g}_{P_i}$
    \STATE $\Theta_{\alpha_i} \gets \Theta_{\alpha_i} - \frac{\eta_t}{L} {\bf g}_{\alpha_i}$

    \STATE Send ${\bf g}_G / L$ to the Federation Server.
    
  \end{algorithmic}
  
  \caption{Alternative Minibatch Update for Mixture of Experts at user $i$ (Outline).}
  \label{alg:2}
\end{algorithm}
\fi


